Investigating the ultraviolet and infrared radiation through the turbulent life of molecular clouds

Context. Molecular Clouds (MCs) are the place where stars are formed and their feedback starts to take place, regulating the evolution of galaxies. Therefore, MCs represent the critical scale at which to study how ultra-violet (UV) photons emitted by young stars are reprocessed in the far-infrared (FIR) by interaction with dust grains, thereby determining the multi-wavelength continuum emission of galaxies. Aims. Our goal is to analyze the UV and IR emission of a MC at different stages of its evolution and relate its absorption and emission properties with its morphology and star formation rate. Such a study is fundamental to determine how the properties of MCs shape the emission from entire galaxies. Method. We consider a radiation-hydrodynamic simulation of a MC with self-consistent chemistry treatment. The MC has a mass $M_{\rm MC} = 10^5 ~ M_\odot$, is resolved down to a scale of $0.06\, \rm pc$, and evolves for $\simeq 2.4$~Myr after the onset of star formation. We post-process the simulation via Monte Carlo radiative transfer calculations to compute the detailed UV-to-FIR emission of the MC. Such results are compared with data from physically-motivated analytical models, other simulations, and observations. Results. We find that the simulated MC is globally UV-optically thick, but optically-thin channels allow for photon escape ($0.1\%-10\%$), feature which is not well-captured in the analytical models. Dust temperature spans a wide range ($T_{\rm dust} \sim 20-300$~K) depending on the dust-to-stellar geometry, which is reproduced reasonably well by analytical models. However, the complexity of the dust temperature distribution is not captured in the analytical models, as evidenced by the 10 K (20 K) difference in the mass (luminosity) average temperature. Indeed, the total IR luminosity is the same in all the models, but the IR emission -abridged

==> include_tex/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother

==> include_tex/pacchetti_mnras.tex <==
\usepackage[english]{babel}
\usepackage{amsmath,amssymb,bm}

\usepackage{graphicx}

\usepackage[normalem]{ulem}

\usepackage{verbatim}
\usepackage{color}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{epstopdf}

\usepackage{url}
\usepackage{xcolor}

\usepackage{gensymb}

\usepackage[usestackEOL]{stackengine}

\usepackage{multirow}

\usepackage{comment}
\usepackage{orcidlink}
